Confidence-Calibrated Adversarial Training: Generalizing to Unseen Attacks

Adversarial training yields robust models against a specific threat model, e.g., $L_\infty$ adversarial examples. Typically robustness does not generalize to previously unseen threat models, e.g., other $L_p$ norms, or larger perturbations. Our confidence-calibrated adversarial training (CCAT) tackles this problem by biasing the model towards low confidence predictions on adversarial examples. By allowing to reject examples with low confidence, robustness generalizes beyond the threat model employed during training. CCAT, trained only on $L_\infty$ adversarial examples, increases robustness against larger $L_\infty$, $L_2$, $L_1$ and $L_0$ attacks, adversarial frames, distal adversarial examples and corrupted examples and yields better clean accuracy compared to adversarial training. For thorough evaluation we developed novel white- and black-box attacks directly attacking CCAT by maximizing confidence. For each threat model, we use $7$ attacks with up to $50$ restarts and $5000$ iterations and report worst-case robust test error, extended to our confidence-thresholded setting, across all attacks.

==> tab_mcifar10_clean_99tpr.tex <==
\begin{tabular}{|@{ }c@{ }|@{ }c@{ }|}
    \hline
    \multicolumn{2}{|c|}{\textbf{CIFAR10:}}\\
    \multicolumn{2}{|c|}{\TE in \%}\\
    \hline
    \hline
    \begin{tabular}{@{}c@{}}$\tau = 0$\end{tabular} &
    \begin{tabular}{@{}c@{}}$99\%$\\TPR\end{tabular}\\
    \hline
    \hline
    \bfseries 8.3 & 7.4\\
    16.6 & 15.5\\
    19.4 & 18.3\\ % \AdvTrainFull
    10.1 & \bfseries 6.7\\
    \hline
    \hline
    18.4 & 17.6\\
    15.2 & 13.2\\ % \TRADES
    %16.9 & 15.2\\ % \WongAT
    13 & 11.7\\ % \MadryAT
    %\hline\hline
    %6.4 & 4.9\\
    \hline
\end{tabular}

==> tab_mcifar10_corrupted2_main_99tpr.tex <==
\begin{tabular}{|@{\hskip 7px}c@{\hskip 7px}|}
\hline
\\
\hline
\hline
\begin{tabular}{@{}c@{}}corr.\\{\tiny CIFAR10-C}\end{tabular}\\
\hline
\textcolor{colorbrewer1}{\bfseries unseen}\\
\hline
\TE$\downarrow$\\
\hline
\hline
12.3\\
16.2\\
19.6\\
8.5\\
\hline\hline
19.3\\
15.0\\
16.8\\
12.9\\
\hline\hline
11.59\\
12.4\\
\hline
\end{tabular}


==> tab_mcifar10_corrupted_main_99tpr.tex <==
\begin{tabular}{|c|}
\hline
\\
\hline
\begin{tabular}{@{}c@{}}corr.\\{\tiny CIFAR10-C}\end{tabular}\\
\hline
\textcolor{colorbrewer1}{\bfseries unseen}\\
\hline
\TE$\downarrow$\\
\hline
\hline
12.3\\ % \Normal 99
16.2\\ % \AdvTrain 99
19.6\\ % \AdvTrainFull 99
8.5\\ % \ConfTrain 99
\hline\hline
19.3\\ % \Wong 99
15.0\\ % \TRADES 99
%16.8\\ % \WongAT 99
12.9\\ % \MadryAT 99
\hline
%11.59\\
%12.4\\
%\hline
\end{tabular}


==> tab_mmnist_corrupted2_main_99tpr.tex <==
\begin{tabular}{|c|}
\hline
\\
\hline
\hline
\begin{tabular}{@{}c@{}}corr.\\{\tiny MNIST-C}\end{tabular}\\
\hline
\textcolor{colorbrewer1}{\bfseries unseen}\\
\hline
\TE$\downarrow$\\
\hline
\hline
32.8\\ % \Normal 99
12.6\\ % \AdvTrain 99
17.6\\ % \AdvTrainFull 99
5.7\\ % \ConfTrain 99
\hline\hline
6.0\\ % \Wong 99
7.9\\ % \TRADES 99
3.3\\ % \WongAT 99
\hline
\end{tabular}


==> tab_mmnist_corrupted_main_99tpr.tex <==
\begin{tabular}{|c|}
\hline
\\
\hline
\begin{tabular}{@{}c@{}}corr.\\{\tiny MNIST-C}\end{tabular}\\
\hline
\textcolor{colorbrewer1}{\bfseries unseen}\\
\hline
\TE$\downarrow$\\
\hline
\hline
32.8\\ % \Normal 99
12.6\\ % \AdvTrain 99
17.6\\ % \AdvTrainFull 99
5.7\\ % \ConfTrain 99
\hline\hline
6.0\\ % \Wong 99
7.9\\ % \TRADES 99
%3.3\\ % \WongAT 99
\hline
\end{tabular}


==> tab_msvhn_clean_99tpr.tex <==
\begin{tabular}{|@{ }c@{ }|@{ }c@{ }|}
    \hline
    \multicolumn{2}{|c|}{\textbf{SVHN:}}\\
    \multicolumn{2}{|c|}{\TE in \%}\\
    \hline
    \hline
    \begin{tabular}{@{}c@{}}$\tau = 0$\end{tabular} &
    \begin{tabular}{@{}c@{}}$99\%$\\TPR\end{tabular}\\
    \hline
    \hline
    3.6 & 2.6\\
    3.4 & 2.5\\
    5.9 & 4.6\\ % \AdvTrainFull
    \bfseries 2.9 & \bfseries 2.1\\
    \hline
    \hline
    \textcolor{gray}{--} & \textcolor{gray}{--}\\ % \Wong
    \textcolor{gray}{--} & \textcolor{gray}{--}\\ % \TRADES
    %\textcolor{gray}{--} & \textcolor{gray}{--}\\ % \WongAT
    \textcolor{gray}{--} & \textcolor{gray}{--}\\ % \MadryAT
    %\hline\hline
    %3.3 & 2.2 \\
    \hline
\end{tabular}
